SCAR: Data Selection via Style Consistency-Aware Response Ranking for Efficient Instruction-Tuning of Large Language Models

Recent studies emphasize that manually ensuring a consistent response style and maintaining high data quality in training sets can significantly improve the performance of fine-tuned Large Language Models (LLMs) while reducing the number of training examples needed. However, the precise definition of style and the relationship between style, data quality, and LLM performance remains unclear. This research identifies two key stylistic elements in responses: linguistic form and instructional surprisal. We find that, among training data of comparable quality, higher consistency in these response elements leads to better LLM performance. Inspired by this, we introduce Style Consistency-Aware Response Ranking (SCAR), which automatically prioritizes instruction-response pairs in the training set based on their response stylistic consistency. By selecting the most style-consistent examples, using only 0.7% of the full dataset in the best case, the fine-tuned LLMs can match or even surpass the performance of models trained on the entire dataset in coding and open-ended question-answering benchmarks. Code and data are available at https://github.com/zhuang-li/SCAR .

==> tab-ablation_llms.tex <==
\begin{table*}[ht!]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|c|ccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Data Sampling} \\ \textbf{Methods}\end{tabular}} & \textbf{HumanEval} & \multicolumn{3}{c}{\textbf{MultiPL-E}} \\
\cdashline{2-5}
& \textbf{Python} & \textbf{Java} & \textbf{JavaScript} & \textbf{C++} \\
& \textbf{Pass@1 / Pass@10} & \textbf{Pass@1 / Pass@10} & \textbf{Pass@1 / Pass@10} & \textbf{Pass@1 / Pass@10} \\
\hline
\multicolumn{5}{c}{Human Data} \\
\hline
GPT-3.5-turbo & & \multicolumn{3}{c}{} \\
\ \ \ \ 50\%  & 32.44 / 50.38 & 30.67 / 44.86 & 34.40 / 53.16 & 29.49 / 45.73 \\
\ \ \ \ 25\%  & 31.98 / 49.25 & 30.41 / 43.65 & 34.04 / 52.72 & 29.19 / 43.41 \\
\ \ \ \ 12.5\%  & 31.10 / 47.14 & 29.46 / 43.06 & 31.38 / 49.11 & 27.61 / 42.39 \\
\hline
Llama-70b & & \multicolumn{3}{c}{} \\
\ \ \ \ 50\%  & 31.21 / 50.01 & 30.14 / 44.23 & 34.67 / 51.90 & 28.67 / 43.90 \\
\ \ \ \ 25\%  & 31.19 / 47.83 & 31.22 / 45.73 & 32.91 / 52.41 & 28.32 / 44.85 \\
\ \ \ \ 12.5\%  & 30.13 / 45.39 & 28.72 / 42.68 & 30.99 / 49.60 & 27.39 / 42.85 \\
\hline
Llama-13b (low thres) & & \multicolumn{3}{c}{} \\
\ \ \ \ 50\%  & 33.60 / 50.02 & 30.47 / 44.53 & 33.88 / 52.96 & 28.91 / 45.22 \\
\ \ \ \ 25\%  & 31.76 / 47.47 & 30.73 / 43.98 & 32.51 / 51.11 & 29.42 / 43.47 \\
\ \ \ \ 12.5\%  & 30.56 / 45.26 & 28.82 / 43.19 & 31.24 / 49.35 & 26.89 / 40.95 \\
\hline
Llama-13b (high thres) & & \multicolumn{3}{c}{} \\
\ \ \ \ 50\%  & 33.60 / 50.02 & 30.47 / 44.53 & 33.88 / 52.96 & 28.91 / 45.22 \\
\ \ \ \ 25\%  & 31.76 / 47.47 & 30.73 / 43.98 & 32.51 / 51.11 & 29.42 / 43.47 \\
\ \ \ \ 12.5\%  & 30.56 / 45.26 & 28.82 / 43.19 & 31.24 / 49.35 & 26.89 / 40.95 \\
\hline
\multicolumn{5}{c}{Mixed Synthetic Data} \\
\hline
Llama-70b & & \multicolumn{3}{c}{} \\
\ \ \ \ 50\%  & 31.21 / 50.01 & 30.14 / 44.23 & 34.67 / 51.90 & 28.67 / 43.90 \\
\ \ \ \ 25\%  & 31.19 / 47.83 & 31.22 / 45.73 & 32.91 / 52.41 & 28.32 / 44.85 \\
\ \ \ \ 12.5\%  & 30.13 / 45.39 & 28.72 / 42.68 & 30.99 / 49.60 & 27.39 / 42.85 \\
\hline
Llama-13b (low thres) & & \multicolumn{3}{c}{} \\
\ \ \ \ 50\%  & 33.60 / 50.02 & 30.47 / 44.53 & 33.88 / 52.96 & 28.91 / 45.22 \\
\ \ \ \ 25\%  & 31.76 / 47.47 & 30.73 / 43.98 & 32.51 / 51.11 & 29.42 / 43.47 \\
\ \ \ \ 12.5\%  & 30.56 / 45.26 & 28.82 / 43.19 & 31.24 / 49.35 & 26.89 / 40.95 \\
\hline
Llama-13b (high thres) & & \multicolumn{3}{c}{} \\
\ \ \ \ 50\%  & 33.60 / 50.02 & 30.47 / 44.53 & 33.88 / 52.96 & 28.91 / 45.22 \\
\ \ \ \ 25\%  & 31.76 / 47.47 & 30.73 / 43.98 & 32.51 / 51.11 & 29.42 / 43.47 \\
\ \ \ \ 12.5\%  & 30.56 / 45.26 & 28.82 / 43.19 & 31.24 / 49.35 & 26.89 / 40.95 \\
\hline
\bottomrule
\end{tabular}
}
\caption{Detailed performance comparison of CodeLlama-7b on the HumanEval (Python) and MultiPL-E (Java, JavaScript, C++) coding benchmarks, fine-tuned with GPT-3.5-generated datasets sampled using different sampling methods in different portions. The Pass@1 and Pass@10 scores for each individual programming language are reported.}
\label{tab:coding_domain_ablation_expanded}
\end{table*}

==> tab-full_results_coding_tab1.tex <==
\begin{table}[ht!]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|c|ccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Data Curation} \\ \textbf{Methods}\end{tabular}} & \textbf{HumanEval} & \multicolumn{3}{c}{\textbf{MultiPL-E}} \\
\cdashline{2-5}
& \textbf{Python} & \textbf{Java} & \textbf{JavaScript} & \textbf{C++} \\
& \textbf{Pass@1 / Pass@10} & \textbf{Pass@1 / Pass@10} & \textbf{Pass@1 / Pass@10} & \textbf{Pass@1 / Pass@10} \\
\hline
\hline
Human Response & 32.93 / 47.93 & 29.78 / 42.35 & 33.84 / 51.85 & 30.05 / 44.38 \\
\hline
\gptThreeFive & & \multicolumn{3}{c}{} \\
\ \ \ \ Referenced & 30.83 / 54.61 & 31.53 / 42.43 & 33.96 / 53.19 & 30.31 / 45.05 \\
\ \ \ \ Direct & 38.95 / 53.82 & 32.11 / 44.49 & 37.86 / 53.97 & 31.52 / 46.45 \\
\hline
\llamaTwoSeventyB & & \multicolumn{3}{c}{} \\
\ \ \ \ Referenced & 30.94 / 48.18 & 29.71 / 41.84 & 32.36 / 52.13 & 27.64 / 43.59 \\
\ \ \ \ Direct & 37.26 / 50.14 & 29.96 / 42.73 & 35.52 / 50.66 & 29.69 / 45.86 \\
\hline
\llamaTwoThirteenB & & \multicolumn{3}{c}{} \\
\ \ \ \ Referenced & 26.20 / 43.52 & 26.65 / 38.45 & 29.02 / 47.91 & 25.63 / 41.60 \\
\ \ \ \ Direct & 26.16 / 39.13 & 22.77 / 33.04 & 28.57 / 43.56 & 23.01 / 35.19 \\
\bottomrule
\end{tabular}
}
\caption{Detailed performance comparison of fine-tuned \codeLlamaSevenB evaluated on HumanEval (Python) and MultiPL-E (Java, JavaScript, C++) coding benchmarks. The LLMs are fine-tuned on training sets curated with different response generation strategies and LLMs. Pass@1 and Pass@10 scores for each programming language are reported.}
\label{tab:coding_domain_expanded}
\end{table}

==> tab-full_style_analysis_tab1.tex <==


% \begin{table}[ht!]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|cc|cc|cc|cc|cc||cc}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Data Curation} \\ \textbf{Methods}\end{tabular}}  & \multicolumn{2}{c|}{\textbf{TTR}} & \multicolumn{2}{c|}{\textbf{MTLD}} & \multicolumn{2}{c|}{\textbf{Avg. Sent. Len.}} & \multicolumn{2}{c|}{\textbf{Punct. Freq.}}  & \multicolumn{2}{c||}{\textbf{Flesch Score}} & \multicolumn{2}{c}{\textbf{Perplexity$(y|x)$}} \\
% \cline{2-13} 
% & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.}  \\
% \hline
% \hline
% \multicolumn{13}{c}{\textbf{StackExchange}} \\
% \hline
% Human Response & 59.36 & 22.27 & 14.65 & 8.57 & 77.77 & 72.59 & 33.12 & 28.42 & 40.84 & 46.78 & 3.33 & 1.41  \\
% \hline
% GPT-3.5-turbo & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}  \\
% \ \ \ \ Referenced & 32.35 & 7.95 & 13.92 & 2.68 & 43.01 & 18.51 & 39.39 & 21.73 & 55.25 & 16.48 & 1.87 & 0.31  \\
% \ \ \ \ Direct & 34.88 & 7.75 & 13.62 & 2.64 & 43.82 & 21.52 & 34.65 & 19.07 & 52.12 & 36.16  & 1.84 & 0.28  \\
% \hline
% Llama2-70b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{}  & \multicolumn{2}{c}{}  \\
% \ \ \ \ Referenced & 43.89 & 11.09 & 14.68 & 3.79 & 59.88 & 39.26 & 34.91 & 24.77 & 52.40 & 20.80 & 2.02 & 0.48 \\
% \ \ \ \ Direct & 44.64 & 12.49 & 14.25 & 3.87 & 64.42 & 53.47 & 31.67 & 24.11 & 51.46 & 21.21& 1.62 & 0.25  \\
% \hline
% Llama2-13b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   \\
% \ \ \ \ Referenced & 31.83 & 7.29 & 15.96 & 3.03 & 38.59 & 17.85 & 46.93 & 26.09 & 61.10 & 15.65 & 1.80 & 0.24 \\
% \ \ \ \ Direct & 31.91 & 8.27 & 15.09 & 3.06 & 40.15 & 26.34 & 40.29 & 23.56 & 59.59 & 16.56 & 1.74 & 0.22 \\
% \hline
% \multicolumn{13}{c}{\textbf{LIMA}} \\
% \hline
% Human Response & 33.26 & 19.54 & 16.39 & 8.98 & 27.19 & 33.89 & 56.99 & 61.87 & 64.93 & 22.89 &8.89 & 8.01  \\
% \hline
% GPT-3.5-turbo & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   \\
% \ \ \ \ Referenced & 47.44 & 17.43 & 15.65 & 5.63 & 24.81 & 16.55 & 14.78 & 10.93 & 57.72 & 21.26 &5.94 & 5.86 \\
% \ \ \ \ Direct & 46.61 & 16.43 & 15.26 & 5.39 & 24.69 & 16.39 & 14.17 & 9.44 & 55.06 & 20.88 &3.19 & 3.61 \\
% \hline
% Llama2-70b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   \\
% \ \ \ \ Referenced & 38.87 & 16.08 & 15.56 & 4.75 & 23.96 & 16.71 & 26.44 & 18.32 & 60.31 & 18.64 & 4.74 & 5.04\\
% \ \ \ \ Direct & 36.50 & 15.60 & 15.34 & 5.14 & 23.66 & 15.43 & 27.74 & 16.67 & 57.83 & 18.32 & 2.51 & 3.11\\
% \hline
% Llama2-13b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{} \\
% \ \ \ \ Referenced & 34.39 & 12.96 & 16.52 & 4.24 & 23.91 & 13.00 & 27.93 & 15.91 & 63.31 & 17.66 & 3.70 & 3.49\\
% \ \ \ \ Direct & 30.63 & 13.18 & 15.57 & 3.93 & 23.62 & 17.88 & 33.87 & 17.39 & 59.85 & 19.11 & 2.41 & 1.13 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Detailed performance comparison of Stylometric Analysis across StackExchange and LIMA datasets showing average and standard deviation for five metrics.}
% \label{tab:style_analysis_expand}
% \end{table}


% \begin{table}[ht!]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|cc|cc|cc|cc|cc||cc|cc|cc}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Data Curation} \\ \textbf{Methods}\end{tabular}}  & \multicolumn{2}{c|}{\textbf{TTR}} & \multicolumn{2}{c|}{\textbf{MTLD}} & \multicolumn{2}{c|}{\textbf{Avg. Sent. Len.}} & \multicolumn{2}{c|}{\textbf{Punct. Freq.}}  & \multicolumn{2}{c||}{\textbf{Flesch Score}} & \multicolumn{2}{c}{\textbf{PPL$(y|x)$}} & \multicolumn{2}{c}{\textbf{PPL$(y_c|x)$}} & \multicolumn{2}{c}{\textbf{GSI}} \\
% \cline{2-17} 
% & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} \\
% \hline
% \hline
% \multicolumn{17}{c}{\textbf{StackExchange}} \\
% \hline
% Human Response & 59.36 & 22.27 & 14.65 & 8.57 & 77.77 & 72.59 & 33.12 & 28.42 & 40.84 & 46.78 & 3.33 & 1.41 & 2.43 & 0.99 & Z.ZZ & W.WW \\
% \hline
% GPT-3.5-turbo & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
% \ \ \ \ Referenced & 32.35 & 7.95 & 13.92 & 2.68 & 43.01 & 18.51 & 39.39 & 21.73 & 55.25 & 16.48 & 1.87 & 0.31 & 1.86 & 0.57 & C.CC & D.DD \\
% \ \ \ \ Direct & 34.88 & 7.75 & 13.62 & 2.64 & 43.82 & 21.52 & 34.65 & 19.07 & 52.12 & 36.16  & 1.84 & 0.28 & 1.86 & 0.55 & G.GG & H.HH \\
% \hline
% Llama2-70b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
% \ \ \ \ Referenced & 43.89 & 11.09 & 14.68 & 3.79 & 59.88 & 39.26 & 34.91 & 24.77 & 52.40 & 20.80 & 2.02 & 0.48 & 2.04 & 0.80 & K.KK & L.LL \\
% \ \ \ \ Direct & 44.64 & 12.49 & 14.25 & 3.87 & 64.42 & 53.47 & 31.67 & 24.11 & 51.46 & 21.21 & 1.62 & 0.25 & 1.64 & 0.45 & O.OO & P.PP \\
% \hline
% Llama2-13b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
% \ \ \ \ Referenced & 31.83 & 7.29 & 15.96 & 3.03 & 38.59 & 17.85 & 46.93 & 26.09 & 61.10 & 15.65 & 1.80 & 0.24 & 1.93 & 0.64 & S.SS & T.TT \\
% \ \ \ \ Direct & 31.91 & 8.27 & 15.09 & 3.06 & 40.15 & 26.34 & 40.29 & 23.56 & 59.59 & 16.56 & 1.74 & 0.22 & 1.93 & 0.63 & W.WW & X.XX \\
% \hline
% \multicolumn{17}{c}{\textbf{LIMA}} \\
% \hline
% Human Response & 33.26 & 19.54 & 16.39 & 8.98 & 27.19 & 33.89 & 56.99 & 61.87 & 64.93 & 22.89 &8.89 & 8.01 & 92.72 & 71.28 & AA.AA & BB.BB \\
% \hline
% GPT-3.5-turbo & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
% \ \ \ \ Referenced & 47.44 & 17.43 & 15.65 & 5.63 & 24.81 & 16.55 & 14.78 & 10.93 & 57.72 & 21.26 &5.94 & 5.86 & 76.88 & 53.19 & EE.EE & FF.FF \\
% \ \ \ \ Direct & 46.61 & 16.43 & 15.26 & 5.39 & 24.69 & 16.39 & 14.17 & 9.44 & 55.06 & 20.88 &3.19 & 3.61 & 42.65 & 28.28 & II.II & JJ.JJ \\
% \hline
% Llama2-70b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
% \ \ \ \ Referenced & 38.87 & 16.08 & 15.56 & 4.75 & 23.96 & 16.71 & 26.44 & 18.32 & 60.31 & 18.64 & 4.74 & 5.04 & 52.60 & 33.37 & MM.MM & NN.NN \\
% \ \ \ \ Direct & 36.50 & 15.60 & 15.34 & 5.14 & 23.66 & 15.43 & 27.74 & 16.67 & 57.83 & 18.32 & 2.51 & 3.11 & 28.06 & 16.08 & QQ.QQ & RR.RR \\
% \hline
% Llama2-13b-chat & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
% \ \ \ \ Referenced & 34.39 & 12.96 & 16.52 & 4.24 & 23.91 & 13.00 & 27.93 & 15.91 & 63.31 & 17.66 & 3.70 & 3.49 & 45.36 & 30.53 & UU.UU & VV.VV \\
% \ \ \ \ Direct & 30.63 & 13.18 & 15.57 & 3.93 & 23.62 & 17.88 & 33.87 & 17.39 & 59.85 & 19.11 & 2.41 & 1.13 & 25.26 & 15.86 & YY.YY & ZZ.ZZ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Detailed performance comparison of Stylometric Analysis across StackExchange and LIMA datasets showing average and standard deviation for five metrics, Perplexity$(y|x)$, Perplexity$(y_c|x)$, and Good’s Surprise Index (GSI).}
% \label{tab:style_analysis_expand}
% \end{table}

\begin{table}[ht!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc||cc|cc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Data Curation} \\ \textbf{Methods}\end{tabular}}  & \multicolumn{2}{c|}{\textbf{TTR}} & \multicolumn{2}{c|}{\textbf{MTLD}} & \multicolumn{2}{c|}{\textbf{Avg. Sent. Len.}} & \multicolumn{2}{c|}{\textbf{Punct. Freq.}}  & \multicolumn{2}{c||}{\textbf{Flesch Score}} & \multicolumn{2}{c}{\textbf{PPL$(y|x)$}} & \multicolumn{2}{c}{\textbf{PPL$(y_c|x)$}} \\
\cline{2-15} 
& \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} \\
\hline
\hline
\multicolumn{15}{c}{\textbf{StackExchange}} \\
\hline
Human Response & 59.36 & 22.27 & 14.65 & 8.57 & 77.77 & 72.59 & 33.12 & 28.42 & 40.84 & 46.78 & 3.33 & 1.41 & 2.43 & 0.99 \\
\hline
\gptThreeFive & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}  & \multicolumn{2}{c}{} \\
\ \ \ \ Referenced & 32.35 & 7.95 & 13.92 & 2.68 & 43.01 & 18.51 & 39.39 & 21.73 & 55.25 & 16.48 & 1.87 & 0.31 & 1.86 & 0.57 \\
\ \ \ \ Direct & 34.88 & 7.75 & 13.62 & 2.64 & 43.82 & 21.52 & 34.65 & 19.07 & 52.12 & 36.16  & 1.84 & 0.28 & 1.86 & 0.55 \\
\hline
\llamaTwoSeventyB & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{}  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
\ \ \ \ Referenced & 43.89 & 11.09 & 14.68 & 3.79 & 59.88 & 39.26 & 34.91 & 24.77 & 52.40 & 20.80 & 2.02 & 0.48 & 2.04 & 0.80 \\
\ \ \ \ Direct & 44.64 & 12.49 & 14.25 & 3.87 & 64.42 & 53.47 & 31.67 & 24.11 & 51.46 & 21.21 & 1.62 & 0.25 & 1.64 & 0.45 \\
\hline
\llamaTwoThirteenB & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{} \\
\ \ \ \ Referenced & 31.83 & 7.29 & 15.96 & 3.03 & 38.59 & 17.85 & 46.93 & 26.09 & 61.10 & 15.65 & 1.80 & 0.24 & 1.93 & 0.64 \\
\ \ \ \ Direct & 31.91 & 8.27 & 15.09 & 3.06 & 40.15 & 26.34 & 40.29 & 23.56 & 59.59 & 16.56 & 1.74 & 0.22 & 1.93 & 0.63 \\
\hline
\multicolumn{15}{c}{\textbf{LIMA}} \\
\hline
Human Response & 33.26 & 19.54 & 16.39 & 8.98 & 27.19 & 33.89 & 56.99 & 61.87 & 64.93 & 22.89 &8.89 & 8.01 & 92.72 & 71.28 \\
\hline
\gptThreeFive & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{} \\
\ \ \ \ Referenced & 47.44 & 17.43 & 15.65 & 5.63 & 24.81 & 16.55 & 14.78 & 10.93 & 57.72 & 21.26 &5.94 & 5.86 & 76.88 & 53.19 \\
\ \ \ \ Direct & 46.61 & 16.43 & 15.26 & 5.39 & 24.69 & 16.39 & 14.17 & 9.44 & 55.06 & 20.88 &3.19 & 3.61 & 42.65 & 28.28 \\
\hline
\llamaTwoSeventyB & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{} \\
\ \ \ \ Referenced & 38.87 & 16.08 & 15.56 & 4.75 & 23.96 & 16.71 & 26.44 & 18.32 & 60.31 & 18.64 & 4.74 & 5.04 & 52.60 & 33.37 \\
\ \ \ \ Direct & 36.50 & 15.60 & 15.34 & 5.14 & 23.66 & 15.43 & 27.74 & 16.67 & 57.83 & 18.32 & 2.51 & 3.11 & 28.06 & 16.08 \\
\hline
\llamaTwoThirteenB & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\
\ \ \ \ Referenced & 34.39 & 12.96 & 16.52 & 4.24 & 23.91 & 13.00 & 27.93 & 15.91 & 63.31 & 17.66 & 3.70 & 3.49 & 45.36 & 30.53 \\
\ \ \ \ Direct & 30.63 & 13.18 & 15.57 & 3.93 & 23.62 & 17.88 & 33.87 & 17.39 & 59.85 & 19.11 & 2.41 & 1.13 & 25.26 & 15.86 \\
\bottomrule
\end{tabular}
}
\caption{Comprehensive performance comparison of stylometric analysis across datasets using instructions from StackExchange and LIMA, paired with responses generated by human writers and various LLMs, presenting the average (Mean) and standard deviation (Std.) for five authorship detection metrics, as well as Perplexity$(y_c|x)$ and Perplexity$(y|x)$.}
\label{tab:style_analysis_expand}
\end{table}




